Generative Semantic Segmentation

We present Generative Semantic Segmentation (GSS), a generative learning approach for semantic segmentation. Uniquely, we cast semantic segmentation as an image-conditioned mask generation problem. This is achieved by replacing the conventional per-pixel discriminative learning with a latent prior learning process. Specifically, we model the variational posterior distribution of latent variables given the segmentation mask. To that end, the segmentation mask is expressed with a special type of image (dubbed as maskige). This posterior distribution allows to generate segmentation masks unconditionally. To achieve semantic segmentation on a given image, we further introduce a conditioning network. It is optimized by minimizing the divergence between the posterior distribution of maskige (i.e., segmentation masks) and the latent prior distribution of input training images. Extensive experiments on standard benchmarks show that our GSS can perform competitively to prior art alternatives in the standard semantic segmentation setting, whilst achieving a new state of the art in the more challenging cross-domain setting.

==> tables/ablation_on_color_patch.tex <==
\begin{table}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on color-to-category converter.} Performance on Cityscapes {\tt val} split (mIoU), ADE20K {\tt val} split (mIoU) and MSeg {\tt test} split ($h. mean$) under different category converter approaches..
}
\vspace{-0.4cm}
\renewcommand\tabcolsep{5.9pt}
\renewcommand\arraystretch{1.2}
\small
\begin{center}
 
\begin{tabular}{l|ccc}
\hline

\hline

\hline

\hline
{Form of converter} & {Cityscapes} & {~ADE20K~} & {~~~MSeg~~~} \\
\hline

\hline
Color-pixel mapping&\textcolor{red}{78.4}&46.29&58.95\\
\rowcolor[gray]{.9}
Color-patch mapping&\textbf{\textcolor{red}{79.9}}&\textbf{48.39}&\textbf{61.86}\\

\hline

\hline

\hline

\hline
\end{tabular}
\end{center}
\label{tab:color_patch}
\end{table}

==> tables/ablation_on_tokenization.tex <==
\begin{table}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on structure of VQVAE} The 'maskige' reconstruction performance (mIoU) on Cityscapes semantic {\tt val} split and ADE20k {\tt val} split under different VQVAE structure.
\textit{Pretrain} means which work pretrained the corresponding VQVAE.
\textit{With Maskige} means we project mask into 'maskige' introduced in Section~\ref{sec:maskige} while \textit{without Maskige} means we directly reconstruct mask with $K$ channels.
Unit for \textit{training time} is in GPU hours.
}
\vspace{-0.4cm}
\renewcommand\tabcolsep{3.1pt}
\renewcommand\arraystretch{1.2}
\small
\begin{center}
 
\begin{tabular}{lc|ccc}
\hline

\hline

\hline

\hline
{Pretrain} & {'Maskige'?} & {Cityscapes} & {ADE20K} & Training Time \\
\hline

\hline
Taming-ADE~\cite{esser2021taming}& & - & 32.22  \\
Taming-ImageNet~\cite{esser2021taming} &~\checkmark& 75.09 & 42.70 \\
UViM~\cite{kolesnikov2022uvim}\ & &89.14 & 78.98  \\
\rowcolor[gray]{.9}
DALL$\cdot$E~\cite{ramesh2021zero} &~\checkmark & \textbf{95.17} & \textbf{87.73} \\

\hline

\hline

\hline

\hline
\end{tabular}
\end{center}
\label{tab:converter}
\end{table}

==> tables/ablation_study.tex <==
\begin{table}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on mask-image prior learning} The mIoU~($\%$) and mAcc~($\%$) are  evaluated on the {\tt val} split of ADE20K. `UAI' denotes unlabeled area inpainting, and `TD' denotes Transformer decoder layer. `$d$' is the downsample ratio of token resolution to input image resolution, including 1/8 and 1/4.
}

\vspace{-0.4cm}
\renewcommand\tabcolsep{14.4pt}
\renewcommand\arraystretch{1.2}
\small
\begin{center}
 
\begin{tabular}{lll|cc}
\hline

\hline

\hline

\hline
$d$&UAI& TD &  ~{mIoU}~ & ~{mAcc}~ \\
\hline

\hline
1/8 &&&  42.52 & 52.05 \\ 
1/8 &\checkmark&&  43.33 & 55.30 \\ 
1/4&\checkmark& &   43.66 & 55.69 \\ 
\rowcolor[gray]{.9}
1/4&\checkmark& \checkmark &  \textbf{46.29} & \textbf{57.84} \\ 

\hline

\hline

\hline

\hline
\end{tabular}
\end{center}
\label{tab:converter}
\end{table}

==> tables/comparison_with_same_backbone.tex <==
\begin{table}[t]
\vspace{0.5em}
\tablestyle{1.8pt}{1.1}
\renewcommand\tabcolsep{7.4pt}
\renewcommand\arraystretch{1.1}
\begin{tabular}{x{24}x{42}x{60}|cc}
\hline

\hline

\hline

\hline
Method &  Backbone & Iteration & mIoU \\
\shline
\multicolumn{1}{l}{UperNet~[\textcolor{green}{44}]}& ResNet-101&  80k&\textbf{80.1}\\
\multicolumn{1}{l}{Deeplab V3+~[\textcolor{green}{6}]}& ResNet-101&  80k&79.9\\
\multicolumn{1}{l}{Maskformer~[\textcolor{green}{10}]} &  ResNet-101 & 90k &78.5\\
\multicolumn{1}{l}{Mask2former~[\textcolor{green}{F}]} & ResNet-101 &90k& \textbf{80.1}\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model~(Ours)}& ResNet-101 &80k& 78.5 \\
\shline
\multicolumn{1}{l}{UperNet~[\textcolor{green}{44}]} & Swin-Large &80k&  82.7\\
\multicolumn{1}{l}{Mask2former~[\textcolor{green}{F}]} & Swin-Large &90k& \textbf{83.3}\\
\multicolumn{1}{l}{UViM$^\dag$~[\textcolor{green}{25}]} & Swin-Large &160k& 77.8\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model~(Ours)}& Swin-Large &56k& 79.8\\ 
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model~(Ours)}& Swin-Large &80k& 80.1\\ 
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model~(Ours)}& Swin-Large &90k& 80.2\\ 
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model~(Ours)}& Swin-Large &160k& 81.0 \\ 

\hline

\hline

\hline

\hline
\end{tabular}
\vspace{-0.5em}
\caption{\textbf{Single scale test on Cityscapes {\tt val} split.} 
Swin-Large is pre-trained on ImageNet-22K. GSS refers to GSS-CW variant. UViM$^\dag$~[\textcolor{green}{25}] is reimplemented by us on MMSegmentation~[\textcolor{green}{11}]
}
% \vspace{-0.5em}
\label{tab:comparision_with_same_backbone}
\end{table}

==> tables/comparison_with_same_backbone_cityscapes.tex <==
\begin{table}[tb]
\tablestyle{1.8pt}{1.1}
\renewcommand\tabcolsep{5.9pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{x{24}x{42}x{70}|cc}
\hline

\hline

\hline

\hline
Method &  Backbone & Iteration(batch size) & mIoU \\
\shline
\multicolumn{3}{l}{\emph{- Cityscapes:}}\\
\shline
\multicolumn{1}{l}{UperNet& ResNet-101  &80k&\textbf{80.1}\\
\multicolumn{1}{l}{Deeplab V3+~\cite{chen2018encoder}}& ResNet-101&  80k&79.9\\
\multicolumn{1}{l}{Maskformer~\cite{cheng2021per}} &  ResNet-101 & 90k &78.5\\
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}} & ResNet-101 &90k& \textbf{80.1}\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& ResNet-101 &80k& 78.3 \\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& ResNet-101 &90k&  \\
\shline
\multicolumn{1}{l}{UperNet~\cite{xiao2018unified}} & Swin-Large$\dag$ &~80k~&  \\
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}} & Swin-Large$\dag$ &90k& \textbf{83.3}\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &27.9k(bs=$4\times8$)& 79.6\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &80k(bs=$2\times8$)& 79.7\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &90k(bs=$2\times8$)& \\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &160k(bs=$2\times8$)& \\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &160k(bs=$2\times16$)& 80.6 \\
\shline
\multicolumn{3}{l}{\emph{- ADE20K:}}\\
\shline
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}} & Swin-Large$\dag$ &160k& \textbf{56.1}\\
\rowcolor[gray]{.9}
\multicolumn{1}{l}{\model-CW}& Swin-Large$\dag$ &160k& 48.39 \\
\shline

\hline

\hline

\hline

\hline
\end{tabular}
% \vspace{-1em}
\caption{\textbf{Performance on Cityscapes {\tt val} split  and ADE20K {\tt val} split with ResNet-101 and Swin-Large backbone.} 
$\dag$: Backbone pre-trained on ImageNet-22K. 
}
% \vspace{-1em}
\label{tab:comparision_with_same_backbone_cityscapes}
\end{table}

==> tables/correct_pixel_mask.tex <==
\begin{table}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on Correct pixel mask:} Performance on Cityscapes semantic segmentation {\tt val} split under different token process approaches for the area with correct pixel-wise segmentation prediction.
}
\small
\begin{center}
 
\begin{tabular}{l|cc}
\hline

\hline

\hline

\hline
{Method} & {Cityscapes mIoU(\%)$\uparrow$} & {ADE20K mIoU$\uparrow$} \\
\hline

\hline
w/o Any process & x & x \\
Set to GT & x & x \\
\rowcolor[gray]{.9}
\textbf{Ignore} & \textbf{x} & \textbf{x} \\
\hline

\hline

\hline

\hline
\end{tabular}
\end{center}
\label{tab:converter}
\end{table}

==> tables/depth_estimation.tex <==
\begin{table}[htb]
\tablestyle{1.8pt}{1.05}

\renewcommand\tabcolsep{4.3pt}
\renewcommand\arraystretch{1.2}
\small
\begin{center}
 
\begin{tabular}{l|cc|cc}
\hline

\hline

\hline

\hline
Method & 
PAD-Net~\cite{xu2018pad} &  
MS-CRF~\cite{xu2017multi} & 
UViM~\cite{kolesnikov2022uvim} & 
\model{}-B \\
\hline

\hline
RMSE &
0.792 &
0.586 &
0.467 &
0.594 \\

\hline

\hline

\hline

\hline
\end{tabular}
\end{center}
% \vspace{-1em}
\caption{
\textbf{Performance on depth estimation on NYU-Depth V2:} The Root Mean Square Error (RMSE) is evaluated on the NYU Depth V2 dataset {\tt val} split.
}
% \vspace{-1em}
\label{tab:depth_estimation}
\end{table}

==> tables/mseg_with_same_backbone.tex <==
\begin{table}[t]
\tablestyle{3.8pt}{1.05}
\centering
\renewcommand\tabcolsep{1.8pt}
\renewcommand\arraystretch{1.1}
\small
\begin{tabular}{l|cccccc|c}
\hline

\hline

\hline

\hline
% Method & Backbone & Iteration&VOC~\cite{everingham2010pascal} & Context~\cite{mottaghi2014role} & CamVid~\cite{brostow2009semantic} & WildDash~\cite{zendel2018wilddash}   & KITTI~\cite{geiger2013vision}  & ScanNet~\cite{dai2017scannet} & \textit{h.\ mean} \\
{Method} & VOC & Context & C.V. & W.D.  & KITTI & ScanNet & \textit{h.\ mean} \\
\hline

\hline
\multicolumn{4}{l}{\emph{- HRNet-W48 backbone:}}\\
\shline
MSeg$^\dag$~[\textcolor{green}{26}]   & 63.8& \textbf{39.6} & 73.9 & 60.9 & 65.1 & \textbf{43.5} & 54.9\\
\rowcolor[gray]{.9}
\model~(Ours) & \textbf{65.2}&  38.8& \textbf{75.2}& \textbf{62.5}& \textbf{66.2}&43.1& \textbf{55.2}\\ % slide
\hline

\hline
\multicolumn{5}{l}{\emph{- Swin-Large backbone:}}\\
 \shline
MSeg$^\dag$~[\textcolor{green}{26}]& 78.7 & 47.5 & 75.1 &\textbf{66.1} & 68.1 & 49.0 & 61.7 \\
\rowcolor[gray]{.9}
\model~(Ours) &  $  \textbf{79.2} $ & $  47.5 $ & $\textbf{76.0}$ & $65.0$ & $  \textbf{68.4} $ & $  \textbf{49.8} $ & $\textbf{61.9}$\\
\hline

\hline

\hline

\hline

\end{tabular}
\vspace{-0.5em}
\caption{Cross domain semantic segmentation on MSeg dataset {\tt test} split. \textbf{All results are under the setting of 160k iterations.} MSeg$^\dag$~[\textcolor{green}{26}] is reproduced by us on MMSegmentation~[\textcolor{green}{11}]. 
}
\label{tab:mseg_with_same_backbone}
\vspace{-0.5em}
\end{table}

==> tables/train_cost.tex <==
\begin{table}[tb]
\tablestyle{1.8pt}{1.1}
\renewcommand\tabcolsep{15.5pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{x{24}|ccc}
\hline

\hline

\hline

\hline
iteration & 40k & 80k & 160k \\
\shline
mIoU & & & \\
\hline

\hline

\hline

\hline
\end{tabular}
% \vspace{-1em}
\caption{\textbf{Ablation on shared Transformer encoder and shared {\tt Maskiage}. Experiments conducted on cityscapes dataset}
}
% \vspace{-1em}
\label{tab:train_cost}
\end{table}
